A unified recipe for deriving (time-uniform) PAC-Bayes bounds

We present a unified framework for deriving PAC-Bayesian generalization bounds. Unlike most previous literature on this topic, our bounds are anytime-valid (i.e., time-uniform), meaning that they hold at all stopping times, not only for a fixed sample size. Our approach combines four tools in the following order: (a) nonnegative supermartingales or reverse submartingales, (b) the method of mixtures, (c) the Donsker-Varadhan formula (or other convex duality principles), and (d) Ville's inequality. Our main result is a PAC-Bayes theorem which holds for a wide class of discrete stochastic processes. We show how this result implies time-uniform versions of well-known classical PAC-Bayes bounds, such as those of Seeger, McAllester, Maurer, and Catoni, in addition to many recent bounds. We also present several novel bounds. Our framework also enables us to relax traditional assumptions; in particular, we consider nonstationary loss functions and non-i.i.d. data. In sum, we unify the derivation of past bounds and ease the search for future bounds: one may simply check if our supermartingale or submartingale conditions are met and, if so, be guaranteed a (time-uniform) PAC-Bayes bound.

==> old.tex <==
Consider $X_1, X_2, \dots, X_n \iid P$. Let $\Theta$ be some (measurable) space of parameters. The risk is defined by $R_n(\theta) = \frac{1}{n}\sum_{i=1}^n f(X_i, \theta)$ where $f$ is some loss function. We are interested in minimizing $\Exp[ f(X, \theta)  ]$ w.r.t. $\theta$.

The classical PAC-Bayesian theory goes as follows. Let us define
\begin{equation}
    W_n(\lambda, \theta) = n \left\{ - \log \Exp[ \exp(\lambda f(X, \theta))]  + \lambda R_n(\theta) \right\}.
\end{equation}
Then $\Exp [\exp(W_n(\lambda, \theta))] = 1$.  Now, let $\Mspace{\Theta}$ be the space of probability measures over $\Theta$.




(todo: empirical bernstein)

(todo: style: Optionally stopped PAC-Bayes)



\begin{proposition}[PAC-Bayesian principle] \normalfont
Let $\nu \in \Mspace{\Theta}$.
\begin{equation}\label{eqn:pacbayesprinc}
    \Exp  \exp \left\{ \sup_{\rho \in \Mspace{\Theta} } \int_{\Theta} W_n(\lambda, \theta) \rho(\d \theta) - \kl(\rho \| \nu)  \right\} \le 1.
\end{equation}
%\ben{This prop only relies on $W_n(\lambda,\theta)$ being measurable and $\Exp_{X\sim P}[\exp(W_n(\lambda,\theta))]\le 1$. }
\end{proposition}

\begin{proof}
We fix $X_1, \dots, X_n$ (this is important -- see Remark 1) and define the measure $\nu_{\exp}$ by
\begin{equation}
\frac{\d \nu_{\exp}}{\d \nu}(\theta) \propto \exp(W_n(\lambda, \theta)) .
\end{equation}
Let $Z = \int_\Theta \exp (W_n(\lambda, \theta)) \nu(\d \theta) $. We see that,
\begin{align}
    & \kl(\rho \| \nu) - \kl(\rho \| \nu_{\exp})
    \\
    = & \int_{\Theta} \left\{ \log\left( \frac{\d \rho}{\d \nu} \right) - \log\left( \frac{\d \rho}{\d \nu_{\exp}} \right) \right\} \d\rho
    \\
    = & \int_{\Theta} \log\left( \frac{\d \nu_{\exp}}{\d \nu} \right) \d\rho =  \int_{\Theta} \log \left(\frac{ \exp(W_n(\lambda, \theta))}{Z}\right) \rho(\d \theta)
    \\
    = & \int_{\Theta} W_n(\lambda, \theta) \rho(\d \theta) - \log Z.
\end{align}
Hence,
\begin{equation}\label{eqn:pac-bayesian-identity}
    \int_{\Theta} W_n(\lambda, \theta) \rho(\d \theta) - \kl(\rho \| \nu) = \log \left\{ \int_\Theta \exp (W_n(\lambda, \theta)) \nu(\d \theta)  \right\}  - \kl(\rho \| \nu_{\exp}).
\end{equation}
Hence the supremum in \eqref{eqn:pacbayesprinc} is $\log \left\{ \int_\Theta \exp (W_n(\lambda, \theta)) \nu(\d \theta)  \right\}$, taken iff $\rho = \nu_{\exp}$. Therefore,
\begin{align}
     & \Exp  \exp \left\{ \sup_{\rho \in \Mspace{\Theta} } \int_{\Theta} W_n(\lambda, \theta) \rho(\d \theta) - \kl(\rho \| \nu)  \right\} = \Exp  \left[ \int_\Theta \exp (W_n(\lambda, \theta)) \nu(\d \theta)  \right]
     \\
     = & \int_\Theta \Exp[\exp (W_n(\lambda, \theta))] \nu(\d \theta) = 1.
\end{align} 
\end{proof}

\begin{remark} \normalfont Here the crux of the matter is: (1) $\nu$ is independent of the data. That's why we can use Fubini's theorem to switch the order of integrals. (2) $\rho$ can be data-dependent \emph{since it only appears within the $\Exp$ taken over the randomness over the data} -- which is the case with $\nu_{\exp}$. $\nu_{\exp}$ is a measure instead of a Markov kernel because it happens \emph{within} the $\Exp$.
\end{remark}


The inequality above implies a deviation bound, uniform with respect to the ``pertubation'' of $\theta$.

\begin{theorem}[PAC-Bayesian bound] Let $\nu \in \Mspace{\Theta}$. With probability at least $1-\alpha$, for any measure $\rho \in \Mspace{\Theta}$,
\begin{equation}\label{eqn:pacbayes}
    \frac{\lambda}{n}\sum_{i=1}^n \int_\Theta f(X_i, \theta) \rho(\d \theta) \le \int_{\Theta} \log \Exp[ \exp(\lambda f(X, \theta))] \rho(\d \theta) + \frac{\kl(\rho \| \nu) + \log(1/\alpha)}{n}.
\end{equation}
\end{theorem}
\begin{proof}
Applying Markov's inequality on previous proposition, we get
\begin{equation}
 \text{w.p.}(1-\alpha), \ \forall \rho, \;   \int_{\Theta} W_n(\lambda, \theta) \rho(\d \theta) \le \kl(\rho \| \nu) + \log(1/\alpha).
\end{equation}
Expanding the $W(\lambda, \theta)$ by its definition yields the theorem. 
\end{proof}





Now, let us explore an any-time valid version.

\begin{lemma}[Mixture of martingales] 
\label{lem:mixtures}
Let $\{ \{M_t(\theta)\}_{t \in \mathbb N}: \theta \in \Theta \}$ be a family of martingales (or super/submartingales) on a filtered probability space $(\Omega, \mathcal{A}, \{\mathcal{F}_t\}_{t \in \mathbb N}, \Pr)$, indexed by $\theta$ in a measurable space $(\Theta, \mathcal{B})$ such that:
\begin{itemize}
    \item Each $M_t(\theta)$ is $\mathcal{F}_t\otimes \mathcal{B}$-measurable;
    \item Each $\Exp[ M_t(\theta) | \mathcal{F}_{t-1} ]$ is $\mathcal{F}_{t-1}\otimes \mathcal{B}$-measurable.
\end{itemize}
Let $\mu$ be a %$\sigma$-
finite measure on $(\Theta, \mathcal{B})$ such that for all $t$,
\begin{equation}\label{eqn:l1}
\Pr\otimes\mu\text{-almost everywhere } M_t(\theta) \ge 0   \quad \text{ or} \quad \int \Exp\left[  |M_t(\theta)|   \right] \mu(\d \theta) < \infty.
\end{equation}
Then, the mixture $\{ M^{\mathsf{mix}}_t \}_{t \in \mathbb N}$, where
\begin{equation}
    M^{\mathsf{mix}}_t = \int M_t(\theta) \mu(\d \theta),
\end{equation}
is also a martingale (or super/submartingale).
\end{lemma}
\begin{proof} First consider the case with supermartingales.

Take any $A \in \mathcal{F}_{t-1}$. Since \eqref{eqn:l1}, we can apply Fubini's theorem to $M_t(\theta)$ on $\Pr|_A \otimes \mu$,
\begin{equation}
    \Exp\left[ \id_{A}\int M_t(\theta) \mu(\d \theta) \right] = \int \Exp\left[\id_{A}  M_t(\theta) \right] \mu(\d \theta) =  \int \Exp\left[ \id_A \Exp\left[  M_t(\theta)  \middle\vert \mathcal{F}_{t-1} \right] \right] \mu(\d \theta).
\end{equation}
Next, by \eqref{eqn:l1}, either $\Pr|_A \otimes\mu$-a.e., $\Exp\left[  M_t(\theta)  \middle\vert \mathcal{F}_{t-1} \right] \ge 0$, or
\begin{equation}
  \int \Exp\left[ |\Exp\left[  M_t(\theta)  \mid \mathcal{F}_{t-1} \right]| \right] \mu(\d \theta) \le \int \Exp\left[ \Exp\left[  |M_t(\theta)|  \mid \mathcal{F}_{t-1} \right] \right] \mu(\d \theta) = \int \Exp\left[  |M_t(\theta)|   \right] \mu(\d \theta) < \infty.
\end{equation}
Hence we can apply Fubini's theorem to $\Exp\left[  M_t(\theta)  \middle\vert \mathcal{F}_{t-1} \right]$ on $\Pr|_A \otimes \mu$,
\begin{equation}
    \int \Exp\left[ \id_A \Exp\left[  M_t(\theta)  \middle\vert \mathcal{F}_{t-1} \right] \right] \mu(\d \theta) = \Exp \left[ \id_A \int \Exp\left[  M_t(\theta)  \middle\vert \mathcal{F}_{t-1} \right] \mu(\d \theta)  \right].
\end{equation}
Therefore, we have
\begin{equation}
  \forall A \in \mathcal{F}_{t-1}, \quad  \Exp\left[ \id_{A}\int M_t(\theta) \mu(\d \theta) \right] = \Exp \left[ \id_A \int \Exp\left[  M_t(\theta)  \middle\vert \mathcal{F}_{t-1} \right] \mu(\d \theta)  \right].
\end{equation}
Further, by Fubini's theorem, $\int \Exp\left[  M_t(\theta)  \middle\vert \mathcal{F}_{t-1} \right] \mu(\d \theta)$ is $\mathcal{F}_{t-1}$-measurable. Hence,
\begin{equation}
    \Exp\left[ \int M_t(\theta) \mu(\d \theta) \middle\vert \mathcal{F}_{t-1} \right] =  \int \Exp\left[  M_t(\theta)  \middle\vert \mathcal{F}_{t-1} \right] \mu(\d \theta).
\end{equation}
Therefore, we have
\begin{align}
    \Exp[  M^{\mathsf{mix}}_t | \mathcal{F}_{t-1} ] = \Exp\left[ \int M_t(\theta) \mu(\d \theta) \middle\vert \mathcal{F}_{t-1} \right] =  \int \Exp\left[  M_t(\theta)  \middle\vert \mathcal{F}_{t-1} \right] \mu(\d \theta) \le \int   M_{t-1}(\theta)   \mu(\d \theta) = M^{\mathsf{mix}}_{t-1}.
\end{align}
The fact that $M^{\mathsf{mix}}_t$ is $\mathcal{F}_{t}$-measurable is again guaranteed by Fubini's theorem. Hence $\{ M^{\mathsf{mix}}_t \}$ is a supermartingale.

The case with submartingales can be proven by considering $-M_t(\theta)$. The case with martingales is proven by combining the cases with supermartingales and submartingales.
\end{proof}

\begin{proposition}[PAC-Bayesian martingale] Let $\{ f_t \}$ be a sequence of functions $\cX \times \Theta \to \mathbb R$. Define
\begin{equation}
    W_t(\theta) = \sum_{i=1}^t \left\{ - \log \Expw_{X\sim P}[ \exp( f_i(X, \theta))]  +  f_i(X_i, \theta) \right\} .
\end{equation}
Then, for each $\theta$, $ \{ \exp (W_t( \theta)) \}$ is a nonnegative martingale, and the process
\begin{equation}
    M_t^{\mathsf{PB}} = \exp \left\{  \sup_{\rho \in \Mspace{\Theta} } \left[ \int_{\Theta} W_t(\lambda, \theta) \rho(\d \theta) - \kl(\rho \| \nu) \right] \right\}
\end{equation}
is also a nonnegative martingale.
\end{proposition}
\begin{proof} First note that $ \{ \exp (W_t( \theta)) \}$ is a non-negative martingale.
Hence, due to \eqref{eqn:pac-bayesian-identity},
\begin{align}
    M_t^{\mathsf{PB}} =   \exp \left\{ \sup_{\rho \in \Mspace{\Theta} } \int_{\Theta} W_t(\theta) \rho(\d \theta) - \kl(\rho \| \nu)  \right\} =\int_\Theta \exp (W_t( \theta)) \nu(\d \theta) 
\end{align}
forms a martingale by the previous lemma.
\end{proof}

\begin{theorem}[Anytime valid PAC-Bayesian bound]\label{thm:pac-bayes-anytime} With probability at least $1-\alpha$, for any $t \in \mathbb N^+$ and any probability measure $\rho\in \Mspace{\Theta}$,
\begin{equation}
     \sum_{i=1}^t  \int_{\Theta}   f_i(X_i, \theta) \rho(\d \theta) \le \sum_{i=1}^t \int_{\Theta}  \log \Expw_{X\sim P}[ \exp( f_i(X, \theta))]   \rho(\d \theta) + \kl(\rho \| \nu) + \log(1/\alpha).
\end{equation}
In particular, \eqref{eqn:pacbayes} still holds if $n$ is replaced by any stopping time.
\end{theorem}
\begin{proof}
Applying Ville's inequality to $\{ M_t^{\mathsf{PB}} \}$, we see that, with probability at least $1-\alpha$,
\begin{equation}
    \forall t \in \mathbb N^+, \forall \rho \in \Mspace{\Theta}, \quad  \int_{\Theta} W_t(\theta) \rho(\d \theta) - \kl(\rho \| \nu) \le \log(1/\alpha).
\end{equation}
Expanding $W_t(\theta)$ by its definition yields the desired result.
\end{proof}
\begin{remark}
This is a \emph{linear} bound (or LLN bound). LIL-type may be achieved by stitching.
\end{remark}

\vspace{1in}

Todo:

applications -- (1)  Catoni-Giulini \emph{sequential} confidence region for the mean of random vector. (2) perhaps plug-in CS for mean under bounded kurtosis? (3)...




% OLD SUB-PSI STUFF
 
	
	\subsection{PAC-Bayes templates for sub-$\psi$ processes}
	\label{sec:sub-psi}
	
	We will say that that $(S_t,V_t)$ are sub-$\psi$ if either Definition~\ref{def:sub-psi} or \ref{def:reverse-sub-psi} applies, i.e., they are either forward sub-$\psi$ or reverse sub-$\psi$. 
    In what follows, we will  consider families of sub-$\psi$ processes indexed by some parameter $\theta\in\Theta$. In this case, we will write that $(S_t(\theta),V_t(\theta))$ is a sub-$\psi$ process. This should be taken to mean that, for each fixed $\theta$, $\exp\{\lambda S_t(\theta)-\psi(\lambda)V_t(\theta)\}\leq L_t(\lambda,\theta)$ for an appropriate supermartingale $L_t(\lambda,\theta)$. 
	
	A useful example we encourage the reader to keep in mind is the following. Consider $Z_i$ drawn i.i.d. from $\dist$ with a stationary loss $f$ bounded in $[0,1]$. Let $\mu(\theta) = \E_\dist[f(Z,\theta)]$. Set $S_t(\theta) = t\mu(\theta) - t\hR_t(\theta)$, $V_t(\theta)=t$, and $\psi(\lambda)=\lambda^2/8$.  Hoeffding's lemma implies that \[\E_\dist\exp\{\lambda(\mu(\theta) - f(Z_i,\theta)) - \lambda^2/8\}\leq 1,\] 
	for all $i$. Therefore, by independence and the fact that $f(Z_i,\theta)$ is $\F_{t-1}$ measurable for $i\leq t-1$,  
	\begin{align*}
		\E_\dist[\exp\{\lambda S_t(\theta) - \psi(\lambda) V_t(\theta)\} | \F_{t-1}] &= \prod_{i=1}^t \E_\dist [\exp\{\lambda(\mu(\theta) - f(Z_i,\theta)) - \lambda^2/8\} |\F_{t-1}] \\
		&\leq \prod_{i=1}^{t-1} \exp\{\lambda(\mu(\theta) - f(Z_i,\theta)) - \lambda^2/8\} \\ 
		&= \exp\{\lambda S_{t-1}(\theta) - \psi(\lambda) V_{t-1}(\theta)\},
	\end{align*}
	demonstrating that $(S_t(\theta),V_t(\theta))$ is a sub-$\psi$ process. With this example in hand, we proceed to give a fixed time PAC-bayes bound for sub-$\psi$ processes. 
	
	
	\begin{theorem}[PAC-Bayes for sub-$\psi$ processes]
d		\label{thm:pac-bayes-sub-psi}
		Let $(S_t(\theta),V_t(\theta))$ be a sub-$\psi$ process. Let $\nu\in\Mspace{\Theta}$ be a data-free prior and let $\lambda\in[0,\psi_{\text{max}})$. For each $n$, with probability at least $1-\alpha$ over the sample and all $\rho\in\Mspace{\Theta}$
		\begin{equation}
			\Exp_{\theta\sim\rho}[\lambda S_n(\theta) - \psi(\lambda) V_n(\theta)] \leq \kl(\rho||\nu) + \log(1/\alpha).
		\end{equation}
	\end{theorem}
	\begin{proof}
		By assumption, $\E_{\dist}\exp(\lambda S_t(\theta)-\psi(\lambda) V_t(\theta))\leq \E_\dist L_t(\lambda,\theta)\leq 1$ (where $L_t(\lambda,\theta)$ is either a forward supermartingale or reverse submartingale). Now apply Markov's inequality to Proposition~\ref{prop:pac-bayes-princ}.  
		We obtain that with probability at least $1-\alpha$ over the sample $Z_1,\dots,Z_n$,
		\begin{equation*}
			\exp\bigg\{\sup_\rho \E_{\theta\sim\rho} [\lambda S_t(\theta) - \psi(\lambda) V_t(\theta)] - \kl(\rho||\nu)\bigg\} \leq 1/\alpha. 
		\end{equation*}
		Taking logarithms and rearranging gives the desired result. 
	\end{proof}
	
	
	We present Theorem~\ref{thm:pac-bayes-sub-psi} mainly so that it can be contrasted with the anytime-valid version, which we state as Theorem~\ref{thm:anytime-pac-bayes-sub-psi}. In particular, we draw attention to the fact that the anytime-valid version does not suffer any extra factors in the bound. This underlies the fact that many existing fixed-time PAC-bayes bounds have time-uniform generalizations which suffer no loss of tightness. 
	
	
	\begin{theorem}[Anytime-valid PAC-Bayes for sub-$\psi$ processes]
		\label{thm:anytime-pac-bayes-sub-psi}
		Let $(S_t(\theta),V_t(\theta))$ be a sub-$\psi$ process. Let $\nu\in\Mspace{\Theta}$ be a data-free prior and let $\lambda\in[0,\psi_{\text{max}})$. With probability at least $1-\alpha$ over the sample, for all $t$ and $\rho\in\Mspace{\Theta}$,
		\begin{equation}
			\Exp_{\theta\sim\rho}[\lambda S_t(\theta) - \psi(\lambda) V_t(\theta)] \leq \kl(\rho||\nu) + \log(1/\alpha).
		\end{equation}
	\end{theorem}
	\begin{proof} 
		The proof is similar to that of Theorem~\ref{thm:pac-bayes-sub-psi}, but we employ Ville's inequality instead of Markov's. For a given $\lambda$ and $\theta$, let $L_t(\lambda,\theta)$ be either the supermartingale or reverse-time submartingale which upper bounds $\exp\{\lambda S_t(\theta)-\psi(\lambda) V_t(\theta)\}$. Set 
		\[L_t^{\mix}(\lambda):=\exp\sup_\rho\bigg\{ \E_{\theta\sim\rho}[L_t(\lambda,\theta)] - \kl(\rho||\nu)\bigg\}.\]
		We claim that $L_t^\mix(\lambda)$ is also a supermartingale if $(S_t(\theta),V_t(\theta))$ is a forward sub-$\psi$ process, and a reverse submartingale if $(S_t(\theta),V_t(\theta))$ is a reverse sub-$\psi$ process. Indeed, Lemma~\ref{lem:change-of-measure} gives $L_t^\mix(\lambda) = \E_\nu L_t(\lambda,\theta)$, so $L_t^\mix(\lambda)$ is a mixture of supermartingales or reverse submartingales. Therefore, by Lemma~\ref{lem:mixtures} in Appendix~\ref{app:mixtures}, it is itself a supermartingale or reverse submartingale, respectively. Hence, 
		\begin{align*}
			& \Pr(\exists t\in\N: \exp\sup_\rho\{ \E_{\theta\sim\rho}[\lambda S_t(\theta) - \psi(\lambda) V_t(\theta)] - \kl(\rho||\nu)\}\geq 1/\alpha) \\
			&\leq \Pr(\exists t\in\N: \exp\sup_\rho\{ \E_{\theta\sim\rho}[L_t (\lambda,\theta)] - \kl(\rho||\nu)\}\geq 1/\alpha)\\
			&= 
			\Pr(\exists t\in\N: L_t^{\mix}(\lambda) \geq 1/\alpha) \leq \alpha,
		\end{align*}
		where the first inequality follows by definition of a sub-$\psi$ process, and the final by Ville's inequality (either Theorem~\ref{thm:ville_supermartingales} or \ref{thm:ville_submartingales}), This implies that, with probability at least $1-\alpha$, for all times $t\in\N$ 
		\begin{equation*}
			\exp \sup_{\rho\in\Mspace{\Theta}}\{\E_{\theta\sim\rho}[\lambda S_t(\theta) - \psi(\lambda) V_t(\theta)] - \kl(\rho||\nu)\} \leq 1/\alpha,
		\end{equation*}
		which is as desired. 
	\end{proof}
	
	Like Proposition~\ref{prop:pac-bayes-princ}, we note that Theorems~\ref{thm:pac-bayes-sub-psi} and \ref{thm:anytime-pac-bayes-sub-psi} did not require any distributional assumption on the data. Such assumptions will only be required when constructing sub-$\psi$ process. As such, this opens the door PAC-Bayes bounds for various kinds of dependence. In fact, many of our bounds throughout Sections ~\ref{sec:light-losses} and \ref{sec:heavy-losses} will require no distributional assumptions. 
	












 The notion of a forward sub-$\psi$ process is enough to give a number of anytime-valid PAC-Bayes bounds. Such results can be found in Section~\ref{sec:supermart_bounds} and a summary of which results they generalize in the first row of Table~\ref{tab:generalization}. However, forward sub-$\psi$ processes do not enable us to recover a significant class of existing bounds. For this, we need to resort to reverse submartingales. Accordingly, we introduce the notion of a \emph{reverse} sub-$\psi$ process. 
	

		
	\begin{definition}[Reverse sub-$\psi$ process]
		\label{def:reverse-sub-psi}
		Let $(S_t)_{t=1}^\infty\subset \R$ and $(V_t)_{t=1}^\infty\subset \R_{\geq 0}$ be stochastic processes adapted to a reverse filtration filtration $(\cR_t)_{t=0}^\infty$. For a function $\psi:[0,\psi_{\text{max}})\to \R$, we say $(S_t,V_t)$ is a reverse sub-$\psi$ process if, for every $\lambda\in[0,\psi_{\text{max}})$, there exists some reverse submartingale $(R_t(\lambda))_{t=1}^\infty$ with $R_1(\lambda)\leq 1$ such that, for all $t\geq 1$,
		\begin{equation}
			\exp\{\lambda S_t - \psi(\lambda) V_t\}\leq R_t(\lambda),\; \text{a.s.}
		\end{equation}
	\end{definition}

	Definition~\ref{def:reverse-sub-psi} is very similar to Definition~\ref{def:sub-psi}, except that we are considering reverse time processes and submartingales. 
	Section~\ref{sec:submart_bounds} will demonstrate that for a convex function $g$, $g(\hR_t(\theta))$ is a reverse submartingale with respect to a particular filtration. Therefore, employing the same logic as above, $\E_\dist\exp(\lambda g(\hR_t(\theta)))$ is also a reverse submartingale with respect to this filtration. However, applying Theorem~\ref{thm:ville_submartingales} to this quantity leaves us with the term $\E_\dist \exp(g(\hR_{t_0}(\theta)))$ in the probability bound, for some $t_0$. That is, we obtain that, for any $\alpha\in(0,1)$, $\Pr(\exists t\geq t_0: \exp g(\hR_{t}(\theta)) \geq 1/\alpha) \leq \alpha \E_\dist \exp g(\hR_{t_0}(\theta))$. 
	Instead, we want a term $\psi(\lambda)V_t$ such that $\E_\dist\exp(\lambda g(\hR_{t_0}(\theta)) - \psi(\lambda)V_t)\leq 1$ in order to have no dependence on the process in the bound. 
	
	

















%     \subsection{Application: Anytime confidence spheres}
% 	\label{sec:confidence_sphere}
	
% 	\ben{todo: look over this, fill in assumptions, etc. Also check if any other bounds apply to this setting.}
	
% 	Here we take $\mathcal{X}$ and $\Theta$ both to be $\mathbb R^d$. Let $d$-dimensional random vectors $\Xvec_1, \Xvec_2,\dots \iid P$. Suppose $\Exp[\Xvec] = \muvec$. Let $\rho_{\varthetavec}$ be the normal distribution $\mathcal{N}(\varthetavec, \beta^{-1}\mathbf{I}_d)$. When $\varthetavec \in \sphere$, we have $\kl(\rho_{\varthetavec} | \rho_0) = \beta / 2$.
	
% 	(todo: assumption)
	
% 	Let $\{\lambda_t\}$ be a deterministic sequence of weights. Define
% 	\begin{gather*}
% 		\psi(x)= \min\{x, 1\},
% 		\\
% 		\thres_t(\xvec) = \frac{\psi(\lambda_t \|\xvec\|)}{\lambda_t \|\xvec\|} \xvec, \quad \text{(thresholded sample)}
% 		\\
% 		\muvec_t = \Exp[ \thres_t(\Xvec) ]
% 		\\
% 		f_t(\xvec, \thetavec) = \lambda_t \dotprod{\thetavec}{ \thres_t(\xvec) - \muvec_t }.
% 	\end{gather*}
% 	Note that
% 	\begin{equation*}
% 		\int f_t(\xvec, \thetavec) \rho_{\varthetavec}(\d \thetavec) =  \lambda_t \dotprod{\varthetavec}{ \thres_t(\xvec) - \muvec_t }.
% 	\end{equation*}
% 	Applying our theorem, with probability at least $1-\alpha$, for all $t \in \mathbb N^+$ and all $\varthetavec\in \sphere$,
% 	\begin{equation*}
% 		\sum_{i=1}^t \int f_i(\Xvec_i, \thetavec) \rho_{\varthetavec}(\d \thetavec) \le \sum_{i=1}^t \int  \log \Expw_{\Xvec\sim P}[ \exp( f_i(\Xvec, \thetavec))]   \rho_{\varthetavec}(\d \thetavec) + \kl(\rho_{\varthetavec} \| \rho_0) + \log(1/\alpha),
% 	\end{equation*}
% 	which is,
% 	\begin{equation*}
% 		\sum_{i=1}^t \lambda_i \dotprod{\varthetavec}{ \thres_i(\Xvec_i) - \muvec_i } \le 
% 		\sum_{i=1}^t \int  \log \Expw_{\Xvec\sim P}\left\{ \e^{  \lambda_i \dotprod{\thetavec}{ \thres_i(\Xvec) - \muvec_i }  } \right\}  \rho_{\varthetavec}(\d \thetavec) + \frac{\beta}{2} + \log(1/\alpha).
% 	\end{equation*}
	
	
% 	By Jensen's inequality,
% 	\begin{align*}
% 		&\int  \log \Expw_{\Xvec\sim P}\left\{ \e^{  \lambda_i \dotprod{\thetavec}{ \thres_i(\Xvec) - \muvec_i }  } \right\}  \rho_{\varthetavec}(\d \thetavec)
% 		\\ \le & \log \int \Expw_{\Xvec\sim P}\left\{ \e^{  \lambda_i \dotprod{\thetavec}{ \thres_i(\Xvec) - \muvec_i }  } \right\}  \rho_{\varthetavec}(\d \thetavec)
% 		\\ = & \log \Expw_{\Xvec\sim P}\left\{ \int \e^{  \lambda_i \dotprod{\thetavec}{ \thres_i(\Xvec) - \muvec_i }  } \rho_{\varthetavec}(\d \thetavec) \right\}
% 		\\ & \text{(by Gaussian MGF)}
% 		\\ = & \underbrace{ \log \Expw_{\Xvec\sim P}\left\{ \exp\left(\lambda_i \dotprod{\thetavec}{ \thres_i(\Xvec) - \muvec_i } + \frac{\lambda_i^2}{2\beta} \| \thres_i(\Xvec) - \muvec_i \|^2 \right) \right\} }_{\text{Let's call it }K_i}.
% 	\end{align*}
% 	According to the CG paper,
% 	\begin{equation*}
% 		K_t \lesssim \log(1 + \lambda_t^2 \sigma^2\beta^{-1} + \lambda_t^4 \sigma^4 \beta^{-1}) \le (\lambda_t^2 \sigma^2 + \lambda_t^4 \sigma^4)\beta^{-1} .
% 	\end{equation*}
	
	
	
% 	We thus have the following result.
% 	\begin{lemma}
% 		With probability at least $1-\alpha$, for all $t \in \mathbb N^+$,
% 		\begin{equation}
% 			\left\|  \sum_{i=1}^t \lambda_i (\thres_i(\Xvec_i) - \muvec_i)  \right\| \le \sum_i^t K_i + \frac{\beta}{2} + \log(1/\alpha).
% 		\end{equation}
% 	\end{lemma}
	
% 	Further, according to the CG paper, 
% 	\begin{equation*}
% 		\|\muvec_t - \muvec  \| \lesssim  \lambda_t^2\sigma^2.
% 	\end{equation*}
% 	We thus have the following confidence sphere sequence. 
	
% 	\begin{theorem}With probability at least $1-\alpha$, for all $t \in \mathbb N^+$,
% 		\begin{equation}
% 			\left\| \frac{\sum_{i=1}^t \lambda_i \thres_i(\Xvec_i)}{\sum_{i=1}^t \lambda_i} - \muvec   \right\| \le \frac{\sum_i^t K_i + \frac{\beta}{2} + \log(1/\alpha) + \sum_{i=1}^t \lambda_i\|\muvec_i - \muvec  \| }{\sum_{i=1}^t \lambda_i}.
% 		\end{equation}
% 		In particular, when $\lambda_t \asymp t^{-1/2} \polylog(t) \sigma^{-1}$, the RHS scales as $t^{-1/2} \polylog(t) \sigma$.
% 	\end{theorem}
	
% 	We remark that of all the constants defined in the CG paper, $\lambda$ is the only one that depends on $t$ (which is ``$n$'' in the CG paper). Constants independent of $t$ do not matter and that is why we can say ``according to the CG paper something $\lesssim$ some function of $\lambda_t$'' above.


















% \section{Relationship to fixed-time bounds}
% \label{app:fixed-time-discussion}


% Here we provide a brief discussion on what might be considered a ``fixed-time'' framework for generating PAC-Bayes bounds. For similar frameworks see \citet{begin2016pac} and \citet{rivasplata2020pac}. 
%  The following proposition sits at the heart of many existing results. By leveraging the change of measure formula, it enables us to transform concentration inequalities into PAC-Bayes bounds.
	
	
% 	\begin{proposition}[PAC-Bayesian principle]
% 		\label{prop:pac-bayes-princ}
% 		Let $\nu \in \Mspace{\Theta}$ be a data-free prior. Let   $W(Z^n,\theta)$ be any measurable function such that $\E_\dist\exp(W(Z^n,\theta))\leq 1$. Then, for each $n$, with probability at least $1-\delta$, for all $\rho\in\Mspace{\Theta}$, 
%         \[\E_\rho W(Z^n,\theta) - \kl(\rho||\nu) \leq 1.\]
% 		% \begin{equation}\label{eqn:pacbayesprinc}
% 		% 	\Exp_{\dist} \exp \sup_{\rho \in \Mspace{\Theta}}\bigg\{ \Exp_{\theta\sim\rho} [W_n(Z_1,\dots,Z_n,\theta)] - \kl(\rho \| \nu)  \bigg\} \le 1.
% 		% \end{equation}
% 	\end{proposition}
% 	\begin{proof}
% 		Lemma~\ref{lem:change-of-measure} implies 
% 		\begin{equation*}
% 			\log \E_{\theta\sim\nu} e^{W(Z^n,\theta)} = \sup_{\rho\in\Mspace{\Theta}}\bigg\{\E_{\theta\sim\rho} [W(Z^n,\theta)] - \kl(\rho\|\nu)\bigg\}.
% 		\end{equation*}
% 		Thus, 
% 		\begin{align*}
% 			\E_{\dist}\exp \sup_{\rho}\bigg\{\E_{\rho} [W(Z^n,\theta)] - \kl(\rho\|\nu)\bigg\} &= \E_\dist\E_{\nu} e^{W(Z^n,\theta)} = \E_{\nu}\E_\dist e^{W(Z^n,\theta)} \leq 1,
% 		\end{align*}
% 		where we've used the fact that $\nu$ is independent of the data in order to switch the integrals in the final equality. From here, we apply Markov's inequality to 
% 	\end{proof}
	
	
% 	We can recover various PAC-Bayes bounds via different instantiations of $W_n$ and applying Markov's inequality to Equation~\eqref{eqn:pacbayesprinc}. For instance, Catoni's bound for losses with $\|f\|_\infty\leq 1$ \citep{catoni2003pac} follows by taking $W_n(Z^n,\theta)=\frac{\lambda}{n}\sum_{i=1}^n f(Z_i,\theta)-\lambda\E_\dist[f(Z,\theta)] - \lambda^2/8$. The conditions of the proposition are met since $\E_\dist \exp W_n(Z^n,\theta)\leq 1$ by Hoeffding's lemma. Similarly, McAllester's bound \citep{mcallester1998some} follows by taking $W_n(Z^n,\theta)=2(n-1)[\frac{1}{n}\sum_{i=1}^nf(Z_i,\theta) - \E_\dist f(Z,\theta)]^2 - \log(n).$ This obeys $\E_\dist \exp W_n(Z^n\theta)\leq 1$ via a concentration inequality due to~\cite{seeger2003bayesian}. (McAllester proved the bound in a different way.) 

 
	
% 	It is worth remarking that Proposition~\ref{prop:pac-bayes-princ} does not require that data be drawn i.i.d. from $\dist$ so long as $\exp W_n(X^n,\theta)$ has at most unit expectation. Of course,  many concentration inequalities rely on the i.i.d. assumption. 

